The high-pressure behaviour of 3R-NbS2

The high pressure behaviour of 3R-NbS2 has been investigated by angle-dispersive X-ray powder diffraction using diamond anvil cells up to 14 GPa. The compression behaviour of the structure is highly anisotropic. The compressibility perpendicular to the layers is 2.5 times higher than within the layers. A fit of a 3rd-order Birch-Murnaghan equation of state gave a volume at zero pressure V0=174(1)\AA^3 and a bulk modulus b0=57(1) GPa, with a pressure derivative b'=8.6(5).

==> elements.tex <==
%Zeitschrift fuer Kristallographie, Oldenbourg Muenchen


\renewcommand{\Title}{The high-pressure behaviour of 3R-NbS$\bm{_2}$}        
                   % Footnotenumbers (most strongly discommended) in Title 
                   % have to be constructed. Do not use any footnote command. 
                   

\renewcommand{\AuthorsComplete}{L. Ehm$^*$, K. Knorr and W. Depmeier}   
                   % with all additions (e.g. footnotemarks)
                   % construct footnotemark $^*$ for the corresponding author 
                   % (one only, please!) 
                   % the text appears automatically below first column

\renewcommand{\CorrespondenceAuthor}{(ehm@min.uni-kiel.de)} 
                   % absolutely preferred: (email) only; in round brackets

\renewcommand{\InstitutionOne}{Institut f\"ur Geowissenschaften, Kristallographie, Christian-Albrechts-Universit\"at zu Kiel, D-24098 Kiel}     %will appear under I if more than 1
%\renewcommand{\InstitutionTwo}{}     %will appear under II
%\renewcommand{\InstitutionThree}{}   %will appear under III 
%\renewcommand{\InstitutionFour}{}    %will appear under IV 
%\renewcommand{\InstitutionFive}{}    %will appear under V 
%\renewcommand{\InstitutionSix}{}     %will appear under VI


\renewcommand{\Abstract}{} 
% includes the full abstract in english!


%%%%%%%%%%%%%%%%%%%%%%% for publisher only %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\Paperreceived}{} % date only; format: April 23, 1998
\renewcommand{\Paperaccepted}{} % date only; format: April 24, 1998
\setcounter{Papervolume}{106}   %publisher: volume number here
%\setcounter{page}{XXX}         % publisher: pagenumber here

\renewcommand{\Authors}{} % without any additions for databank purposes

\renewcommand{\cleanTitle}{}   % only needed to eliminate additions from Title 
                               % like footnotes etc. for databank purposes
\renewcommand{\shortAuthors}{} % only needed for headings; else = Authors
\renewcommand{\shortTitle}{}   % only needed for headings; else = cleanTitle
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


